A Review of Bangla Natural Language Processing Tasks and the Utility of Transformer Models

Bangla -- ranked as the 6th most widely spoken language across the world (https://www.ethnologue.com/guides/ethnologue200), with 230 million native speakers -- is still considered as a low-resource language in the natural language processing (NLP) community. With three decades of research, Bangla NLP (BNLP) is still lagging behind mainly due to the scarcity of resources and the challenges that come with it. There is sparse work in different areas of BNLP; however, a thorough survey reporting previous work and recent advances is yet to be done. In this study, we first provide a review of Bangla NLP tasks, resources, and tools available to the research community; we benchmark datasets collected from various platforms for nine NLP tasks using current state-of-the-art algorithms (i.e., transformer-based models). We provide comparative results for the studied NLP tasks by comparing monolingual vs. multilingual models of varying sizes. We report our results using both individual and consolidated datasets and provide data splits for future research. We reviewed a total of 108 papers and conducted 175 sets of experiments. Our results show promising performance using transformer-based models while highlighting the trade-off with computational costs. We hope that such a comprehensive survey will motivate the community to build on and further advance the research on Bangla NLP.

==> sections/_discussions.tex <==
\section{Discussions}
\label{sec:discussions}

\subsection{Discussions: Parts of Speech}
\label{ssec:dis_text_pos}
The transformer based BERT models provide comparable results. Due to BERT tokenizer, our model didn't perform well comparing with resource-rich languages. The bert multilingual pretrained tokenizer breaks most of the Bangla words in subwords, which affected overall performance. Although we used Bangla pretrained BERT tokenizer, the tokenizer doesn't contains all the vocabulary of our dataset. Moreover, our used dataset has english words, which caused low performance of Bangla BERT tokenizer. Comparing with BERT multilingual and BERT Bangla pretrained model, XLM-RoBERTa large pretrained model provide prominent results and outperforms existing PoS tagging results. Although BERT multilingual model accuracy outperforms existing results, yet it has issue with F1 score.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Discussions: Lemmatization}
\label{ssec:dis_text_lemma}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Discussions: Named Entity Recognition}
\label{ssec:dis_text_ner}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Punctuation Restoration}
\label{ssec:dis_punc}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Machine Translation}
\label{ssec:dis_mt}
The transformer based models provide prominent results comparing with other statistical and NMT models. But still it has problems with translating rare words especially the nouns. Increasing in the amount of training data didn't performed as expected due to morphological richness \cite{hasan2020collaborative} and highly-inflected words \cite{hasan2020not}. The translation quality of the test set is not up to the mark \cite{hasan2019neural, hasan2020not} and the training set contains both american and british english, which creates an impact on the overall performance. There is also translation from Indian Bangla to English and some word translations differs from Bangladeshi Bangla (e.g., 'jamuna', 'yamuna'). In figure \ref{fig:mt_ex1}, we present the examples of incorrect translation of the target sentence and appropriate prediction of the model. In our study, we also found that some of the words that have abbreviations (i.e. US Dollar and USD) create an effect on the translation score. In figure \ref{fig:mt_ex3}, we present an example that our system couldn't predict properly. These types of errors are mostly observed in sentences due to the presence of rare words (e.g. {\ban\ পারস্যের} - 'persian', {\ban\ বাবর} - 'babur'). Our study also reveals that the translation of a sentence might be gone entirely wrong in presence of rare words or unknown words.

%\todo{@Arid, please convert these example in image form. We need to arxiv the paper, and bangla text will create problems. You can check how i did for NER, For Bangla text please use solaimanlipi font, copy the example in word then do the necessary formatting and take screenshot.\small use solaimanlipi{}}

\begin{figure}[t]
\centering
\begin{subfigure}{\columnwidth} %[b]{\textwidth}
\centering
    \includegraphics[width=\columnwidth]{figures/mt_ex1.png}
    \includegraphics[width=\columnwidth]{figures/mt_ex2.png}
    % \vspace{-0.9em}
    \caption{Example of wrong predictions by transformer model.}
    \label{fig:mt_ex1}  
    % \vspace{-1.0em}
\end{subfigure}
%\begin{subfigure}{\columnwidth} %[b]{\textwidth}
%\centering
%    \includegraphics[width=\columnwidth]{figures/mt_ex2.png}
%    % \vspace{-0.9em}
%    \caption{Example of wrong predictions by transformer model.}
%    \label{fig:mt_ex2}  
    % \vspace{-1.0em}
%\end{subfigure}
\begin{subfigure}{\columnwidth} %[b]{\textwidth}
\centering
    \includegraphics[width=\columnwidth]{figures/mt_ex3.png}
    % \vspace{-0.9em}
    \caption{Example of few words prediction in a sentence.}
    \label{fig:mt_ex3}  
    % \vspace{-1.0em}
\end{subfigure}
\caption{Example sentences for machine translation}
%\label{fig:rel-acc}  
\vspace{-1.0em}
\end{figure}

%\begin{example}
%\label{mtex_1}
%\small{
%\textbf{Sent:} {\ban\ প্রতিদিন সকালে আমরা দুটি বিস্ময়কর ঘটনা দেখি।}\\
%\textbf{Prediction:} every morning we see two amazing incidents.\\
%\textbf{Target:} every morning we see two wonderful things.
%}
%\end{example}

%\begin{example}
%\label{mtex_2}
%\small{
%\textbf{Sent:} {\ban\ যত বেশী চিৎকার করবে, তত বেশী অনুভব করবে।}\\
%\textbf{Prediction:} the more you scream, the more you feel.\\
%\textbf{Target:} the louder you cry, the more you will feel.
%}
%\end{example}

%\begin{example}
%\label{mtex_3}
%\small{
%\textbf{Sent:} {\ban\ চা বাগান পারস্যের বাগানের মতন করে নকশা করা হয়েছিল যা ভারতে প্রথম করেছিলেন প্রথম মুঘল সম্রাট বাবর।}\\
%\textbf{Prediction:} like the tea garden , the first mughal emperor bakr was designed in india.\\
%\textbf{Target:} the tea garden was designed like a persian %garden , which was first introduced in india by first mughal emperor , babur.
%}
%\end{example}

%চা বাগান পারস্যের বাগানের মতন করে নকশা করা হয়েছিল যা ভারতে প্রথম করেছিলেন প্রথম মুঘল সম্রাট বাবর ।
%T-224	the tea garden was designed like a persian garden , which was first introduced in india by first mughal emperor , babur .
%H-224	like the tea garden , the first mughal emperor bakr was designed in india .

In this study, we also found that the translations of spoken corpora are differs from others corpora. The Tanzil corpus also have translations issues which is not generalize translations and more focusing on religious views. The corpus contains more long sentences, which makes difficulties for learning the parameters while training the transformer models. Tanzil corpus has more Bangla tokens than English comparing with other corpora, which makes the whole training set imbalance.
The training set contains noisy words and covers different domains that create difficulties for the model to predict proper words for the target sequence. Moreover, the GlobalVoices dataset creates difficulties in overall performance because of its long segments, and NMT can't translate properly on long sentence \cite{koehn2017six}. Our reported results on SUPara test set is the second best existing systems. However, reaching the results of resource-rich languages is still a big challenge because of morphological richness, the inflection of words, and low resources. More good quality translations are required to improve on these results for the future.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Discussions: Sentiment Classification}
\label{ssec:dis_text_sentiment}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Emotion Classification}
\label{ssec:dis_emotion}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Authorship identification}
\label{ssec:dis_authorship}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\inote{\textcolor{red}{title would be News Categorization, not Text Categorization}}
\subsection{Discussions: Text Categorization}
\label{ssec:dis_text_categorization}
We can conclude from the results that transformer based models are better suited for Bangla text classification tasks compared to classical machine learning based approaches that use manually engineered features or CNN/LSTM models trained on distributed word representation. We represent the relative accuracy of the three models compared to the best published prior results on each dataset in Figure \ref{fig:rel-acc}. There is a clear trend across the datasets. XLM-RoBERTa-base performs better than BERT and XLM-RoBERTa-large performs better than XLM-RoBERTa-base model. Both XLM-RoBERTa models improve upon previously reported results across all datasets. BERT performs slightly worse than the previous best result on YouTube sentiment-5 class and News sentiment datasets. 

\begin{figure}[t]
\centering
\includegraphics[width=0.8\linewidth]{figures/rel_acc.png}
\vspace{-0.9em}
\caption{Relative accuracy compared to the best published results on different datasets}
\label{fig:rel-acc}  
\vspace{-1.0em}
\end{figure}

There are various factors contributing to the performance gain obtained by XLM-RoBERTa models. They are trained on a larger corpus compared to BERT and has larger vocabulary size. As a result fewer unknown tokens are introduced after tokenization. For example, considering the example sentence from before, we obtain following tokens after using XLM-RoBERTa model tokenizer

\todo{@Akib/Tanvir the following examples need to be converted into image}
{\ban\ '{\_}সুন্দর', '{\_}সব', 'স', 'ময়', '{\_}আনন্দ', 'ময়'}

However, using BERT tokenizer we get the following tokens

{\ban\ 'স', '\#\#ুন', '\#\#্দ', '\#\#র', {\en\ '[UNK]'}, {\en\ '[UNK]'}}

Last two words are replaced with the unknown tokens, even though they are not rare word in Bangla. The first word is also split into several tokens. XLM-RoBERTa performs better in this regard due to availability of larger vocabulary for Bangla in the model. As XLM-RoBERTa-large is a model with trained with more layers and parameters, it also has better generalization ability than XLM-RoBERTa-base model. This results in better performance in the downstream tasks.

One advantage of subword embedding is that it can perform better in noisy user generated text like those found in online media. As they tend to contain misspelling and shortened words, subword embedding (also character embedding) can still capture some meaningful information from them. People also often comment in both Bangla and English in those platforms, as is present in the YouTube datasets. Since we are using multilingual models for fine-tuning which are also trained on large amount of English data, the model is expected to perform better in such cases. This can explain why we got significantly more improvement from transformer models in the YouTube datasets compared to the Bangla news sentiment dataset, which does not contain any English text.

Using transformer models for fine-tuning also reduces the need for feature engineering and data preprocessing. In our experiments, we did not use any separate text preprocessing steps (e.g., stop words and punctuation removal)other than using the model specific tokenizers.
% However, further preprocessing may still yield further improvement and can be explored in future work.

In this experiment, we have explored multilingual language models as they are more readily available, especially for a low resource language like Bangla. If we fine-tune from a monolingual Bangla transformer model pretrained on a large corpus, we believe further improvements can be made on Bangla only texts like in authorship attribution dataset.

\begin{figure}
\centering
\begin{subfigure}{\columnwidth} %[b]{\textwidth}
\centering
    \includegraphics[width=\columnwidth]{figures/sent1.PNG}
    % \vspace{-0.9em}
    \caption{Word importance for sentence{\ban\ 'কেন জানি না! গানটা এতো ভালো লাগে। সবসময় শুনতে ভালো লাগে।'}\textit{ (I don't know why! I like the song so much. Always good to} hear.)  Detected as positive with 0.9972 probability.}
    \label{fig:sent1}  
    % \vspace{-1.0em}
\end{subfigure}
    \hfill
\begin{subfigure}{\columnwidth} 
    \centering
    \includegraphics[width=0.6\columnwidth]{figures/sent2.PNG}
    \caption{Word importance for sentence{\ban\ 'শেষের সিনটা টা খুব খারাপ লেগেছিল}\textit{ (The last scene was very bad!)} Detected as negative with 0.9627 probability.}
    \label{fig:sent2}  
% \vspace{-1.0em}    
\end{subfigure}
\hfill
\begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/sent3.PNG}
    % \vspace{-0.9em}
    \caption{Word importance for sentence{\ban\ 'লাইফে এমন গান খুব কম শুনেছি,হাজার বার শুনেও খারাপ লাগেনি'}\textit{ (I have rarely heard such songs in my life, I have not felt bad even after listening to them a thousand times.}) Detected as positive with 0.9807 probability.}
    \label{fig:sent3}  
% \vspace{-1.0em}  
\end{subfigure}
\caption{Example sentences highlighting the importance of words that network learns.}
\label{fig:example_all}
\end{figure}

% To understand how the model comes at prediction, 
For a better interpretation of the model we explore and show word importance with three example sentences. This is obtained for XLM-RoBERTa large model trained on YouTube sentiment-3 dataset. These representations are produced using Captum \cite{captum2019github}. In Figure \ref{fig:sent1}, the model puts a high emphasis on the positive word {\ban\ ভালো} (good). First sentence {\ban\ কেন জানি না!} (I don't know why!) can be considered to be slightly negative and is reflected in the word importance. In Figure \ref{fig:sent2}, the negative word {\ban\ খারাপ} (bad) is properly highlighted to arrive at the overall negative sentiment. Interestingly {\ban\ খুব} (very) is highlighted as opposite i.e., positive, meaning the model was not able to combine two words and emphasize the phrase {\ban\ খুব খারাপ} (very bad) as negative. Finally, the sentence in Figure \ref{fig:sent3} is more challenging. However the model is able to identify the overall positive tone despite the presence of some negative words like {\ban\ কম, খারাপ} (rarely, bad).



==> sections/introduction.tex <==

\section{Introduction}
\label{sec:intro}

% \inote{\textcolor{red}{TODO: Firoj, Naira, Shammur}}
% \todo[]{Let us maintain American English style.}

% \todo[inline]{@Arid, can you please cite papers on the empty ones in the below paragraph? earlier ref  would be preferable.}
%Changes in Intro by shammur
Bangla is one of the most widely spoken languages in the world~\cite{ali2010unsupervised}, yet it is still considered a low-resource language in terms of digitization, primarily due to the scarcity of annotated computer readable datasets and the limited support for resource building. 
% the fact that resource development support was limited, specifically the development of annotated computer readable datasets. 
Research on Bangla Natural Language Processing (BNLP) began in the early 1990s, with an initial focus on rule-based lexical and morphological analysis \cite{islam2009research,sengupta1993lexical,sengupta1993morpho}. %After the initial stage,
Later the advancement in BNLP research continued in the early 2000s, with a particular focus on Parts of Speech (POS) tagging \cite{hasan2007comparison}, grammar checkers \cite{alam2007n}, Named Entity Recognition (NER) \cite{ekbal2010named,alam2016bidirectional}, morphological analysis \cite{dasgupta2005morphological,dasgupta2004morphological}, parsing using context free grammars\cite{mosaddeque2004context}, Machine Translation (MT)~\cite{sennrich2015neural}, Text-to-Speech (TTS) \cite{alam2007text,alam2008text}, Speech Recognition \cite{hasnat2007isolated,chowdhury2010implementation,paul2009bangla}, and Optical Character Recognition (OCR)~\cite{chaudhuri1998complete,hasnat2008high,hasnat2009open}. 
Over the years, the research focus has extended to include automated text summarization, sentiment analysis \cite{hasan2013sentiment}, emotion detection~\cite{das2010sentiwordnet}, and news categorization~\cite{article}.
%%not new extension, it just continuation
% machine translation~\cite{chatterji2009hybrid}, lemmatization~\cite{chakrabarty2016benlem, chakrabarty2017context}, 
% and news categorization~\cite{article}. %Although Bangla is one of the most widely spoken languages in the world~\cite{ali2010unsupervised}, it is still considered a low-resource language in terms of digitization, primarily due to the fact that resource development support was limited, specifically the development of annotated computer readable datasets. 

% In the early part of the last decade, 

In 2013, a book, highlighting different aspects of Bangla language processing, was complied  \cite{karim2013technical} addressing the limitations as well as the progress made at the time. %In 16 chapters, the aforementioned book presents research on 
The covered content include font design, machine translation, character recognition, parsing, a few avenues of speech processing, information retrieval, and sentiment analysis. Moreover, there have been several endeavors to develop resources and advance the field towards developing machine learning models. However, most of the current research focuses on a finite number of areas, namely, lemmatization, NER, punctuation restoration, and news categorization. 


From the modeling perspective, most of the earlier endeavors are either rule-based,% \cite{hoque2015bangla}, 
statistical or classical machine learning based approaches. Classical machine algorithms include Naive Bayes (NB), Support Vector Machine (SVM) \cite{kudo2001chunking,yamada2003statistical}, and Random Forests (RF)~\cite{breiman2001random} used for the text classification task. As for the sequence tagging tasks, such as NER and G2P, the algorithms include Hidden Markov Models (HMMs) \cite{brants2000tnt}, Conditional Random Fields (CRFs) \cite{lafferty2001conditional}, Maximum Entropy (ME) \cite{ratnaparkhi1996maximum}, Maximum Entropy Markov Models (MEMMs) \cite{mccallum2000maximum}, and  hybrid approach \cite{altun2003hidden}.

Feature engineering has been ubiquitous in earlier days. For text classifications, the features such as token, bag-of-words, and bag-of-n-grams are used to feature representation. In sequence tagging, hand-crafted features include mainly orthographic features such as prefix, suffix, the word in context, abbreviation, and numbers. Task-specific knowledge source such as the lexicon has also been used, which lists whether a word is a noun, pronoun or belongs to some others classes \cite{alam2016bidirectional}.

It is only very recently that a small number of studies have explored deep learning-based approaches 
%\textcolor{red}{PAPERS inBN with DNNs}
\cite{arid2019MTb,AridSentiment2020}, which include Long Short Term Memory (LSTM) neural networks \cite{hochreiter1997long} and Gated Recurrent Unit (GRU) \cite{cho2014learning} and a combination of LSTM, Convolution Neural Networks (CNN) \cite{lecun1989backpropagation} and CRFs \cite{huang2015bidirectional,ma2016end,lample2016neural}. Typically, these algorithms are used with distributed words and character representations called ``word embeddings" and ``character embeddings," respectively. 



% The reported studies for Bangla NER include Ekbal et al. \cite{ekbal2010named,ekbal2009bengali,ekbal2009named,ekbal2008web,ekbal2008development,ekbal2008bengali,ekbal2008named,ekbal2007hidden} and \cite{banerjee2014bengali}.

% The success of both word- and character- level embeddings are reported in many literatures \cite{dos2014learning,ma2016end,lample2016neural,ling2015finding} 

%% resources development
For a low-resource language like Bangla, resource development and benchmarks have been major challenges. At present, publicly available resources are limited %The limited number of datasets that are available include annotated text corpora 
and are focused on certain sets of annotation like  sentiment \cite{tripto2018detecting,ashik2019data}, news categorization data \cite{kunchukuttan2020ai4bharat}, authorship attribution data \cite{khatun2019authorship}, speech corpora \cite{alam2010development,alam2008consacoustic}, parallel corpora for machine translation \cite{hasan2020collaborative,hasan2019icbslp, hasan2019neural}, and pronunciation lexicons \cite{alam2008text,chowdhury2017bangla}. A small number of recent endeavors report benchmarking sentiment and text classification tasks \cite{AridSentiment2020,alam2020bangla}.

% Our motivation for the current paper is 
In this work, we aim to provide a comprehensive survey on the most notable NLP tasks addressed for Bangla, which can help the community with a direction for future research and advance further study in the field.
There has not been any survey on Bangla NLP tasks of this nature; hence this will serve as a first study for the research community. 



Since covering the entire field of Bangla NLP is difficult, we focused on the following tasks: {\em(i)} POS tagging, {\em(ii)} lemmatization, {\em(iii)} NER, {\em(iv)} punctuation restoration, {\em(v)} MT, {\em(vi)} sentiment classification, {\em(vii)} emotion classification, {\em(viii)} authorship attribution, and {\em(ix)} news categorization. %\textcolor{red}{
A recent survey on Bangla language processing reviews the work appeared from 1999 to 2021, where eleven different topics have been addressed in terms of classical to deep learning approaches \cite{sen2021bangla}. Our work differs from theirs as we conduct extensive experiments using nine different transformer models to create benchmarks for nine different tasks. We also conduct extensive reviews on these tasks to compare our results, where possible.
% note to self, rewrite and add more points

% We would like to highlight that covering additional topic on spell checking, parsing, OCR, grammar checker, speech generation would have made this a much stronger resource paper.
% \inote{\textcolor{red}{To Do: Firoj Sir, please read the following contributions. We have only one models for MT, 9 models for sentiment, authorship attribution, news classification, PoS, 8 models for Lemma,}}
In addition to providing a detailed survey on Bangla NLP tasks, we also conducted experiments using the current state-of-the-art pre-trained transformers models on nine different tasks, except the MT task. We provided benchmark results for the research community. To summarize, our contributions in the current study are as follows: 
\begin{enumerate}
    \itemsep0em
    \item A detailed survey on the most notable NLP tasks by reviewing 108 papers.
    \item Experimental results using nine different transformer models for each task, except one model for MT task, which resulted in 175 sets of experiments.
    \item Provide comparative results for different transformer models: (1) large vs. small models, (2) mono vs. multilingual models.
    \item For some tasks, we report comparative results for individual vs. consolidated datasets. 
    \item We analyze the trade-off between performance and computational complexity between the transformer-based and classical approaches like SVM.
    \item Provide a concrete future direction for the community: what resources are available, the challenges, and what can be done.
    \item Provide data splits for reproducibility and future research.\footnote{Note that we could only provide and share data splits, which were publicly accessible. Any private data can be possibly accessed by contacting respective authors.}  
\end{enumerate}

% In this study we presents a literature review and experimental results using transformer models of most of the BNLP research areas. PoS tagging, lemmatization, and NER is consider as essential study in terms of NLP research where the other areas are equally important.


% has been undergone rapid advancement with the emergence of deep neural networks, especially transformer network has been studied in recent years. 

In Section \ref{sec:background}, we provide a background study of different approaches to BNLP, including the research conducted to date. We then describe the pre-trained transformer-based language models \ref{sec:methods}. We proceed to discuss the data and experiments in each area of BNLP in Section \ref{sec:experiments}. We also report the experimental results and discuss our findings \ref{sec:results}. The individual overall performance, limitation, and future work are discussed in Section \ref{sec:challenge_future_work}. Finally, we conclude our study with the future direction of BNLP research in Section \ref{sec:conclusion}.
% \label{sec:challenge_future_work}
% note to self: revise

